Scenario-Based Safety Assessment Framework for Automated Vehicles

Automated vehicles (AVs) are expected to increase traffic safety and traffic efficiency, among others by enabling flexible mobility-on-demand systems. This is particularly important in Singapore, being one of the world's most densely populated countries, which is why the Singaporean authorities are currently actively facilitating the deployment of AVs. As a consequence, however, the need arises for a formal AV road approval procedure. To this end, a safety assessment framework is proposed, which combines aspects of the standardized functional safety design methodology with a traffic scenario-based approach. The latter involves using driving data to extract AV-relevant traffic scenarios. The underlying approach is based on decomposition of scenarios into elementary events, subsequent scenario parametrization, and sampling of the estimated probability density functions of the scenario parameters to create test scenarios. The resulting test scenarios are subsequently employed for virtual testing in a simulation environment and physical testing on a proving ground and in real life. As a result, the proposed assessment pipeline thus provides statistically relevant and quantitative measures for the AV performance in a relatively short time frame due to the simulation-based approach. Ultimately, the proposed methodology provides authorities with a formal road approval procedure for AVs. In particular, the proposed methodology will support the Singaporean Land Transport Authority for road approval of AVs.

==> sections/virtual_safety_validation.tex <==
\section{Virtual safety validation}
\label{sec:virtualSafetyValidation}

The virtual safety validation aims to quantitatively assess the operational safety of AVs in a virtual test environment. Virtual testing allows for a wide variety of test scenarios to be executed, among which scenarios that may not occur in real life very frequently, covering multiple scenario classes with a diversity of activity parameter sets per class.

A schematic of the envisioned simulation architecture is given in Fig.~\ref{fig:simulationSetup}. The scenario database, as indicated in this figure, contains scenarios which are described in terms of activity parameters and scenario tags, jointly referred to as `scenario parameters'. With the scenario parameters as knowledge base, test scenarios are generated by selecting certain types of scenarios using the tagging system and subsequently generating instances of those scenarios by means of drawing samples from the probability distribution of the activity parameters. This step, as indicated in Fig.~\ref{fig:simulationSetup} by the red-dashed block, is part of the \emph{scenario generation} component (see Section~\ref{sec:scenarioGeneration}).

\begin{figure}[tb]
	\centering
	\includegraphics[width=\textwidth]{simulation_setup}
	\caption{High-level structure of simulation setup for virtual safety validation.}
	\label{fig:simulationSetup}
\end{figure}

In the remainder of this section, the scenario information is divided into the following groups:
\begin{itemize}
	\item \emph{Ego vehicle}: the autonomous vehicle-under-test (VUT), i.e., the AV, whose goals are described by the particular test case;
	\item \emph{Dynamic objects}: other road users, whose motions are described by the activity parameters;
	\item \emph{Static objects}: static scenario information that is not subject to significant changes within the time frame of a scenario. Static objects are subsequently divided into:
	\begin{itemize}
		\item \emph{Road topology}: the coordinates of the various roads in the scene with corresponding semantical classification by the scenario tags such as `crossing', `roundabout', and `motorway';
		\item \emph{Scenery}: the environment of the VUT, such as infrastructure, types of roads, road conditions, and type of weather, corresponding to the scenario tags.
	\end{itemize}
\end{itemize}
These scenario parameter groups may not be exhaustive yet, but they are adequate in the scope of the description of the simulation setup.

The parameters of the candidate test scenarios provide the dynamic and static object information that needs to be transformed into simulation inputs and parameters, involving the following operations:
\begin{enumerate}
	\item For each selected test scenario, or set of selected test scenarios, a certain area or road is selected from a digital map, having the characteristics as indicated by the semantic information contained in the tags of those test scenarios. From the road topology in the digital map, \emph{road coordinates} will directly follow. These road coordinates serve as input to the simulation, providing path boundaries for the model of the VUT.
	\item The road coordinates, together with the activity parameters of the test scenario, serve as input for the computation of the \emph{dynamic object trajectories}, which, in turn, are input to the simulation.
	\item \emph{Scenery parameters} are provided to the simulation model, that requires to transform semantic information into numerical simulation parameters. Depending on the level of fidelity of the simulation environment, weather conditions, such as rain and sunlight, may be included in the simulation.
	\item \emph{Ego vehicle parameters} are provided to the VUT model, describing the role of the VUT in the scenario in terms of, e.g., desired route, maximum speed, and certain assignments such as a forced lane change. In addition, the type of VUT, such as `passenger car', `bus', or 'van', or even the detailed vehicle model parameters may be prescribed.        
\end{enumerate}
These operations, which are captured in the green-dashed block in Fig.~\ref{fig:simulationSetup}, require a simulation environment which is capable of defining a detailed road topology and scenery, such as CarMaker.

Having defined ego vehicle parameters, dynamic object trajectories, road coordinates, and scenery parameters as inputs, the actual simulation involves, firstly, creating inputs for the VUT sensor models. To this end, the absolute position, velocity, and acceleration of all dynamic objects, and the position of all static objects (insofar applicable) must be transformed to a vehicle-fixed VUT coordinate frame, thus providing ground-truth inputs for the VUT environment sensors. The last part of the simulation setup is then the VUT model itself, which incorporates dynamic models of the vehicle and its sensor system, the sensor fusion algortihms, and the control system algorithms, the latter being `instructed' by the ego vehicle parameters from the test scenario. Obviously, to properly assess the behavior of the VUT, the sensor models should include typical uncertainties, such as noise, multipath and other inherent impairments. Moreover, it must be possible to inject component failures in order to test functional safety aspects. The coordinate transformation and the dynamic model of the VUT are indicated by the blue-dashed block in Fig.~\ref{fig:simulationSetup}. %Since a detailed simulation model of the VUT must be included, software tools such as CarMaker and the M\textsc{atlab}/Simulink-based simulation tool PreScan are suitable.
CarMaker is used to provide a detailed simulation model of the VUT.

\begin{remark}
	The scheme of Fig.~\ref{fig:simulationSetup} has an important inherent limitation, being the fact that the trajectories of the dynamic objects are chosen \textit{a priori}, such that these objects will not react to VUT behavior in any way. Although this approach may be adequate for many test scenarios, at some point in the future, it may be required to model true interaction between other road users and the VUT. In terms of the block scheme, this can be implemented by including multiple instances of road user models, following the same setup as the VUT model, but with known behavior. Consequently, a \emph{multi-agent simulation} arises.
\end{remark}

%\begin{remark}
%	The AV simulation model, including the vehicle platform and sensor parameters, and the perception and control software, can be provided by the AV developer. Alternatively, these simulation modules are provided by CETRAN as part of the assessment pipeline. Either way, the quality of this model, and particularly the quality of the sensor models, must be sufficiently high to obtain reliable simulation results. To this end, CETRAN currently already investigates the use of validated error models, combined with a relatively simple (non-physical) sensor model. It is proposed to investigate the desired simulation setup as well as adequate model quality measures together with one or several AV developers.
%\end{remark}

